Parallel Algorithms for Summing Floating-Point Numbers

The problem of exactly summing n floating-point numbers is a fundamental problem that has many applications in large-scale simulations and computational geometry. Unfortunately, due to the round-off error in standard floating-point operations, this problem becomes very challenging. Moreover, all existing solutions rely on sequential algorithms which cannot scale to the huge datasets that need to be processed. In this paper, we provide several efficient parallel algorithms for summing n floating point numbers, so as to produce a faithfully rounded floating-point representation of the sum. We present algorithms in PRAM, external-memory, and MapReduce models, and we also provide an experimental analysis of our MapReduce algorithms, due to their simplicity and practical efficiency.

==> approx.tex <==

\paragraph{Summation Tree}
This version of the floating-point summation problem is to
constructing a summation tree, $T$, having
the elements of $X$ associated with its leaves (in some order)
such
that each internal node, $v$ in $T$, represents the floating-point addition,
\[
x_v^*=x_u^*\oplus x_w^*,
\]
of the (recursively-computed) 
floating-point values, $x_u^*$ and $x_w^*$, 
respectively associated with $v$'s two children, $u$ and $w$.  
Thus, when computed (in parallel as a bottom-up
computation), the root, $r$, of $T$ will store $x_r^*=S_n^*$.

Following the problem formulation of Kao and 
Wang~\cite{doi:10.1137/S0097539798341594},
the optimization goal in this problem is to construct $T$ so as 
to minimize the total \emph{worst-case}
error, $E(T)$, for $T$, 
which is defined as
\[
E(T) = \alpha \sum_{{\rm internal}\ v\in T} x_v,
\]
where $x_v$ is the true summation value for the numbers stored in 
the leaves of $v$'s subtree in $T$, where $v$ is an internal node in $T$
(and $\alpha$ is the machine-dependent roundoff error bound for
floating-point addition).
This minimization is taken over all possible summation trees for the
numbers in $X$.

The summation-tree floating-point summation problem is
motivated especially by the problem of summing $n$ arbitrary-precision
floating-point numbers, where exact computations would be potentially space
inefficient.
We are interested in the following two versions of this problem:
\begin{itemize}
\item
\emph{Single-sign Summation Tree.}
In this problem, all the numbers in $X$ have the same sign---positive
or negative.
\item
\emph{Mixed-sign Summation Tree.}
In this problem, the numbers in $X$ include at least one positive
number and at least one negative number.
\end{itemize}
Designing
efficient parallel algorithms for 
these two versions of the summation-tree problem poses interesting challenges,
because the optimal solution to the single-sign summation tree
problem is a 
Huffman tree (which, in general, will not have $O(\log n)$ depth)
and computing an optimal solution for the mixed-sign summation tree
problem is NP-hard~\cite{doi:10.1137/S0097539798341594}.


